Spiral of Silence in Large Language Model Agents

The Spiral of Silence (SoS) theory holds that individuals with minority views often refrain from speaking out for fear of social isolation, enabling majority positions to dominate public discourse. When the 'agents' are large language models (LLMs), however, the classical psychological explanation is not directly applicable, since SoS was developed for human societies. This raises a central question: can SoS-like dynamics nevertheless emerge from purely statistical language generation in LLM collectives? We propose an evaluation framework for examining SoS in LLM agents. Specifically, we consider four controlled conditions that systematically vary the availability of 'History' and 'Persona' signals. Opinion dynamics are assessed using trend tests such as Mann-Kendall and Spearman's rank, along with concentration measures including kurtosis and interquartile range. Experiments across open-source and closed-source models show that history and persona together produce strong majority dominance and replicate SoS patterns; history signals alone induce strong anchoring; and persona signals alone foster diverse but uncorrelated opinions, indicating that without historical anchoring, SoS dynamics cannot emerge. The work bridges computational sociology and responsible AI design, highlighting the need to monitor and mitigate emergent conformity in LLM-agent systems.

==> analysis_discussion.tex <==
% !TEX root = acl_latex.tex
\section{Analysis and Discussion}

Based on the experimental results in table \ref{tab:qwen}, \ref{tab:llama}, 
we conducted further analysis of these results. In addition, due to space limitations, Figures \ref{fig:qwen_prompt_a} to \ref{fig:llama_hard100} have been placed in the appendix.

\subsection{Consistent vs. Inconsistent Across Different Datasets}

\textbf{GSM8K Dataset.} GSM8K (Grade School Math 8K) contains 8,000 math problems, primarily covering basic arithmetic, algebra, and simple geometry. The problems are typically word problems and application-based, suitable for elementary to middle school students.
Due to the relatively simple and structured nature of the problems, models show higher consistency between self-assessment and problem-solving ability on the GSM8K dataset. The models can better make self-assessment, leading to better alignment between self-assessment and actual problem-solving ability, especially on Easy100 compared to Hard100.


\noindent\textbf{MATH and Math500 Datasets.} The MATH dataset includes 6,000 challenging math problems, covering advanced topics such as algebra, calculus, combinatorics, and linear algebra. The Math500 dataset includes 500 problems from a wide range of mathematical areas, including algebra, geometry, and probability, with varying levels of difficulty. Compared to GSM8K, the problems in the MATH and Math500 datasets are more complex and require deeper mathematical knowledge. Models tend to struggle with self-assessment when solving these more difficult problems, often leading to inconsistencies between their self-assessment and actual problem-solving ability. The complexity of these problems makes it harder for models to accurately assess their difficulty, resulting in discrepancies.

\subsection{Differences in Consistency Between Llama Variant Models and Qwen Series Models}

The Qwen series models show better consistency between self-assessment and problem-solving ability compared to the GSM8K dataset. Specifically, models fine-tuned for mathematical tasks exhibit stronger problem-solving capabilities than those not fine-tuned for such tasks. As shown in Figures \ref{fig:qwen_prompt_a} and \ref{fig:qwen_prompt_b}, Qwen2.5-Math-1.5B-Instruct outperforms Qwen2.5-7B-Instruct, and Qwen2.5-Math-7B-Instruct outperforms Qwen2.5-1.5B-Instruct, demonstrating a significant improvement in problem-solving ability due to fine-tuning for mathematical tasks. On datasets like GSM8K and Math500, the Qwen models consistently perform well, with better stability and alignment between self-assessment and problem-solving ability, likely due to their fine-tuning on mathematical tasks.

In contrast, the Llama variant models exhibit lower consistency between self-assessment and problem-solving ability. These models have not been fine-tuned for mathematical tasks, which contributes to greater discrepancies in their self-assessments and problem-solving ability, particularly on more complex mathematical problems.

\subsection{The Influence of Model Size}

As shown in Figures \ref{fig:qwen_prompt_a} and \ref{fig:qwen_prompt_b}, the problem-solving capability of Qwen2.5-7B-Instruct consistently outperforms that of Qwen2.5-1.5B-Instruct. Similarly, Qwen2.5-Math-7B-Instruct demonstrates superior problem-solving ability over Qwen2.5-Math-1.5B-Instruct in most cases. Figures \ref{fig:llama_prompt_a} and \ref{fig:llama_prompt_b} further illustrate that Llama-3.2-3B-Instruct consistently outperforms Llama-3.2-1B-Instruct. Additionally, despite minor differences between Llama-3.3-70B-Instruct and its Llama-3.2 counterparts (Llama-3.2-1B-Instruct and Llama-3.2-3B-Instruct), the significantly larger scale of Llama-3.3-70B-Instruct ensures its superior problem-solving capability in all cases.

\subsection{The Impact of Structured Promptings}

Structured prompting methods have a significant impact on model performance, especially for more complex mathematical problems. Well-designed prompts help guide the model to better understand the problem, leading to more accurate reasoning and solutions.
In both Qwen series and Llama variant models, adjusting the prompting configuration helps the model adapt better to problems of varying difficulty. For harder problems, optimized prompting methods assist in more accurate self-assessment, which improves the consistency between self-assessment and problem-solving ability.

As shown in Figure \ref{fig:qwen_easy100}, the Qwen series models exhibit better problem-solving ability on Easy100 with prompt B. Similarly, Figure \ref{fig:llama_hard100} shows that the Llama variant models perform better on Hard100 with prompt B. Additionally, Figure \ref{fig:qwen_hard100} illustrates the superior problem-solving ability of the Qwen series models on Hard100 with prompt A, while Figure \ref{fig:llama_easy100} shows that the Llama variant models excel on Easy100 with prompt A.


==> preliminaries.tex <==
% !TEX root = acl_latex.tex
%\section{Prelinaries}
\section{Approach}
\subsection{Problem Setup}
We simulate a population of LLM agents tasked with rating movies under controlled conditions to examine SoS dynamics.
Consider an online rating system with a set of LLM agents and a set of items.
Each agent evaluates the quality of items based on an $M-$level cardinal rating metric denoted by 
$\mathcal{M}
\stackrel{\triangle}{=}
\{1,\ldots, M\}$, 
where $M \in \mathbb{N}_{+}$. 
The rating given by agent $i$ to item $j$ is denoted by $r_{i,j} \in \mathcal{M}$.
A higher rating reflects a stronger preference of the agent toward the item.
As an illustration, when $M = 10$, the scale can be interpreted as $\mathcal{M} \stackrel{\triangle}{=}$ \{1 = ``\texttt{Awful/Abysmal}'', $\cdots$,
5 = ``\texttt{Mediocre/Unsure}'', $\cdots$, 10 = ``\texttt{Perfect/Masterpiece}''\}. 



\paragraph{Collective opinion.}
Let $r_{j,k} \in \mathcal{M}$ denote the $k$-th observed rating of item $j$,
where $k \in \mathbb{N}_{+}$. let $\mathcal{H}_{j,k}$ denote a set of 
all historical ratings of item j up to the $k$-th rating, formally: 
\begin{align*}
&
\mathcal{H}_{j,k}
\stackrel{\triangle}{=} 
\left\{ 
r_{j,1}, \ldots, r_{j,k} 
\right\},
&&
\forall k \in \mathbb{N}_+.
\end{align*}

Now, we model the formation of collective opinions, that is, the function $\mathcal{F} ( \mathcal{H}_{j,k} )$.  
agents may form a climate of opinions from the aggregation of historical ratings.
Denote the collective opinion summarized from the rating history $\mathcal{H}_{j,k}$ as 
\[
\bm{h}_{j,k}
\!\stackrel{\triangle}{=}\!
[h_{i, k, 1}, \ldots, h_{j, k, M}], 
\]
where $h_{j,k,m} \in [0,1]$ and 
$\sum_{m \in \mathcal{M}} h_{j,k,m} =1$.   
The $\bm{h}_{j,k}$ is public to all agents.  
We consider a \textit{class} of weighted aggregation rules
to summarize historical ratings: 
\begin{align}
& 
h_{j, k, m} =
\frac{\sum^k_{l = 1} \alpha_j \mathbb{I}_{\{r_{j,l} = m\}}}{\sum^k_{l =1} \alpha_l},
&& 
\forall m \in \mathcal{M}, k \in \mathbb{N}_+
\end{align}

\noindent where $\alpha_l \in \mathbb{R}_+$ denotes 
the weight associated with $k$-th rating,
and $\mathbb{I}$ is an indicator function.  
For example, $\alpha_j \!=\! 1, \forall j$, is deployed in many rating systems, 
which corresponds to ``\textit{average rating rule}''.  
Under this average rating rule, we have 
$
h_{j, k, m}
\!=\!
\sum^k_{l=1} \mathbb{I}_{\{R_{j,l} = m\}} / k
$, which is the fraction of historical ratings equal to $m$.  
Note that $\bm{h}_{j,k}$ is displayed to all agents.  
We capture the collective opinion formation as follows:  
\begin{align}
\mathcal{F} ( \mathcal{H}_{j,k} )
= \sum_{ m \in \mathcal{M} } m \cdot h_{j,k,m} 
\end{align}

==> result.tex <==
% !TEX root = acl_latex.tex
\section{Results}




\begin{table*}[h]
    \centering
    \small
    \caption{
    The results of the Qwen2.5 series models are presented, where the symbol \greensquare indicates alignment between self-assessment and problem-solving capabilities, and the symbol \redtriangle signifies a misalignment between self-assessment and problem-solving abilities.
    }
    \label{tab:qwen}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccc}
        \toprule
        \textbf{Model} &
        \textbf{Prompt} &
        \textbf{Subset} & 
        \textbf{MATH} & &
        \textbf{Maht500} & &
        \textbf{GSM8K} & \\
        \midrule
        Qwen2.5-1.5B-Instruct & prompt A & Easy100 & 0.46 & \redtriangle & 0.35 & \redtriangle & 0.66 & \redtriangle \\
        & & Hard100 & 0.65 & & 0.38 & & 0.77 & \\
        \midrule
        Qwen2.5-1.5B-Instruct & prompt B & Easy100 & 0.42 & \redtriangle & 0.53 & \redtriangle & 0.69 & \redtriangle\\
        & & Hard100 & 0.49 & & 0.53 & & 0.75 &\\
        \midrule
        Qwen2.5-Math-1.5B-Instruct& prompt A & Easy100 & 0.55 & \redtriangle & 0.71 & \redtriangle & 0.93 & \greensquare\\
        & & Hard100 & 0.72 & & 0.76 & & 0.73 &\\
        \midrule
        Qwen2.5-Math-1.5B-Instruct & prompt B & Easy100 & 0.50 & \redtriangle & 0.73 & \greensquare & 0.81 & \greensquare\\
        & & Hard100 & 0.64 & & 0.68 & & 0.74 &\\
        \midrule
        Qwen2.5-7B-Instruct& prompt A & Easy100 & 0.71 & \redtriangle & 0.76 & \redtriangle & 0.92 & \redtriangle\\
        & & Hard100 & 0.80 & & 0.84 & & 0.93 &\\
        \midrule
        Qwen2.5-7B-Instruct& prompt B & Easy100 & 0.45 & \redtriangle & 0.53 & \redtriangle & 0.93 & \greensquare\\
        & & Hard100 & 0.83 & & 0.85 & & 0.89 &\\
        \midrule
        Qwen2.5-Math-7B-Instruct & prompt A & Easy100 & 0.91 & \greensquare & 0.93 & \greensquare & 0.97 & \greensquare\\
        & & Hard100 & 0.55 & & 0.68 & & 0.88 &\\
        \midrule
        Qwen2.5-Math-7B-Instruct& prompt B & Easy100 & 0.71 & \redtriangle & 0.72 & \redtriangle & 0.98 & \greensquare\\
        & & Hard100 & 0.77 & & 0.86 & & 0.89 & \\
        \midrule
        Qwen2.5-72B-Instruct& prompt A & Easy100 & 0.57 & \redtriangle & 0.68 & \redtriangle & 0.87 & \redtriangle\\
        & & Hard100 & 0.82 & & 0.86 & & 0.87 &\\
        \midrule
        Qwen2.5-72B-Instruct& prompt B & Easy100 & 0.59 & \redtriangle & 0.73 & \redtriangle & 0.88 & \greensquare\\
        & & Hard100 & 0.81 & & 0.82 & & 0.84 &\\
        \bottomrule
    \end{tabular}
    }
\end{table*}

\noindent\textbf{Qwen Series Models.} According to the experimental results presented in Table \ref{tab:qwen}, for Qwen series models, an intriguing phenomenon was observed. On the MATH dataset, among the ten results corresponding to five models and two prompt configurations, only the Qwen2.5-Math-7B-Instruct model demonstrated consistency between self-assessment and problem-solving capability when using self-assessment prompt A, with higher accuracy on Easy100 compared to Hard100. On the Math500 dataset, similar to the results on the MATH dataset, consistency between self-assessment and problem-solving capability was only observed in the Qwen2.5-Math-1.5B-Instruct model using self-assessment prompt B and the Qwen2.5-Math-7B-Instruct model using self-assessment prompt A. But on the GSM8K dataset, stronger alignment between self-assessment and problem-solving capability was observed. In two mathematically fine-tuned models, consistency between self-assessment and problem-solving capability was achieved under different prompt configurations, and the Qwen2.5-7B-Instruct model also demonstrated this alignment when using self-assessment prompt B. These phenomena suggest that models may exhibit a difficulty assessment bias, where they fail to accurately assess the difficulty of the problems. %\zy{GSM8K is naturally easier than MATH and MATH500? so the self-assessment can hold in the easier dataset?}



Further analysis of the results from the MATH and Math500 datasets reveals that different prompts impact the consistency between self-assessment and problem-solving capability. Specifically, the Qwen2.5-Math-7B-Instruct model demonstrated alignment between self-assessment and problem-solving capability when using self-assessment prompt A, but showed misalignment when using self-assessment prompt B.

Additionally, we found that mathematically fine-tuned models outperform non-fine-tuned models in terms of problem-solving accuracy and the consistency between self-assessment and problem-solving capability, suggesting that fine-tuning helps models better assess the difficulty of mathematical problems and enhances overall performance.

Finally, in most cases, the Qwen2.5-7B-Instruct model outperforms the Qwen2.5-1.5B-Instruct model in terms of problem-solving accuracy, and the Qwen2.5-Math-7B-Instruct model outperforms the Qwen2.5-Math-1.5B-Instruct model in accuracy as well. This suggests that model size positively influences problem-solving ability, with larger models being better suited for handling complex mathematical reasoning tasks.

\begin{table*}[h]
    \centering
    \caption{The results of the Llama variant models are presented, where the symbol \greensquare indicates alignment between self-assessment and problem-solving capabilities, and the symbol \redtriangle signifies a misalignment between self-assessment and problem-solving abilities.}
    \label{tab:llama}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccccc}
        \toprule
        \textbf{Model} &
        \textbf{Prompt} &
        \textbf{Subset} & 
        \textbf{MATH} & &
        \textbf{Maht500} & &
        \textbf{GSM8K} & \\
        \midrule
        Llama-3.2-1B-Instruct& prompt A & Easy100  & 0.01 & \redtriangle & 0.09 & \redtriangle & 0.19 & \redtriangle \\
        & & Hard100  & 0.27 & & 0.24 & & 0.34 & \\
        \midrule
        Llama-3.2-1B-Instruct & prompt B & Easy100  & 0.18 & \redtriangle & 0.22 & \redtriangle & 0.29 & \redtriangle\\
        & & Hard100  & 0.27 & & 0.24 & & 0.31 &\\
        \midrule
        Llama-3.2-3B-Instruct & prompt A & Easy100  & 0.17 & \redtriangle & 0.25 & \redtriangle & 0.70 & \redtriangle\\
        & & Hard100  & 0.67 & & 0.73 & & 0.82 & \\
        \midrule
        Llama-3.2-3B-Instruct & prompt B & Easy100  & 0.33 & \redtriangle & 0.43 & \redtriangle & 0.71 & \greensquare\\
        & & Hard100 & 0.52 & & 0.59 & & 0.87 &\\
        \midrule
        Llama-3.3-70B-Instruct & prompt A & Easy100  & 0.42 & \redtriangle & 0.52 & \redtriangle & 0.96 & \redtriangle \\
        & & Hard100  & 0.80 & & 0.88 & & 0.93 &\\
        \midrule
        Llama-3.3-70B-Instruct & prompt B & Easy100  & 0.35 & \redtriangle & 0.53 & \redtriangle & 0.96 & \redtriangle\\
        & & Hard100  & 0.78 & & 0.84 & & 0.98 & \\
        \bottomrule
    \end{tabular}%
    }
\end{table*}

\noindent\textbf{Llama Variant Models.} According to the experimental results presented in Table \ref{tab:qwen}, for the Llama variant models, it is surprising that, among the six results corresponding to three models and two prompt configurations across three datasets, only the Llama-3.2-3B-Instruct model demonstrated consistency between self-assessment and problem-solving capability when using self-assessment prompt B. This phenomenon suggests that the consistency between self-assessment and problem-solving capability in Llama variant models may be problematic, raising concerns about their overall alignment across tasks.

Further analysis, similar to the results observed in the Qwen series models, indicates that the choice of prompt significantly affects the consistency between self-assessment and problem-solving capability. Notably, model size has a positive impact on problem-solving ability, with larger models better equipped to handle complex mathematical reasoning tasks. Therefore, model size may be a crucial factor influencing the consistency of these abilities.

Additionally, it is important to note that we did not use Llama variant models that have been fine-tuned for mathematical tasks, which could be one of the reasons for the lower overall consistency between self-assessment and problem-solving capability in the Llama variant models compared to the Qwen series models.


